Temporal mixture ensemble models for intraday volume forecasting in cryptocurrency exchange markets

We study the problem of the intraday short-term volume forecasting in cryptocurrency exchange markets. The predictions are built by using transaction and order book data from different markets where the exchange takes place. Methodologically, we propose a temporal mixture ensemble, capable of adaptively exploiting, for the forecasting, different sources of data and providing a volume point estimate, as well as its uncertainty. We provide evidence of the outperformance of our model by comparing its outcomes with those obtained with different time series and machine learning methods. Finally, we discuss the predictions conditional to volume and we find that also in this case machine learning methods outperform econometric models.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> backup.tex <==
% \begin{equation}
% \text{IW} = \frac{1}{C} \sum (y^{+}_{i} - y^{-}_{i}),
% \end{equation}
% \begin{equation}
% \text{IW} = \frac{1}{N} \sum_{i=1}^M (y^{+}_{i} - y^{-}_{i})= \frac{1}{N} \sum_{i=1}^M{4\hat{\sigma}_i},
% \end{equation}
% \begin{equation}
% \text{IW} = \frac{1}{C} \sum_{y_i \in [y^{-}, y^{+}]} (y^{+}_{i} - y^{-}_{i})= \frac{1}{C} \sum_{y_i \in [y^{-}, y^{+}]}{4\hat{\sigma}_i},
% \end{equation}
% The IW measure should be minimized and it tells that the high-quality prediction intervals should be as narrow as possible, while capturing a specified portion of data, without assumptions on the distribution \cite{pearce2018high}.
% The Pearson correlation coefficient between the predicted volume and true volume is: %E[(v_t-E[v_t]) (\hat{v}_t-E[\hat{v}_t])] / \sigma[v_t] \sigma[\hat{v}_t]
% \begin{equation}
% \text{CORR} = \frac{\sum_{i=1}^M (y_i-E[y_i])(\hat{y}_i-E[\hat{y}_i])}
% {\sqrt{\sum_{i=1}^M(y_t-E[y_i])^2} \sqrt{\sum_{i=1}^M(\hat{y}_i-E[\hat{y}_i])^2}}
% \end{equation}
% and clearly larger values indicate better models.
% this type of metric evaluates how well the distribution characterized by predictive mean $\hat{y}_i$ and variance $\hat{\sigma}_i^2$ fits the ground-truth target values.
% The $2 \hat{\sigma}$ coverage (IC) counts the fraction of true values $y_i$ that fall within $2\hat{\sigma}_i$ range, where $\hat{\sigma}_i$ is the predictive standard deviation:
% \begin{equation}
% \text{IC} = \frac{1}{M} \sum_{i=1}^{M} \textbf{1}_{[\hat{y}_i-2\hat{\sigma}_i \leq y_i \leq \hat{y}_i+2\hat{\sigma}_i]}.
% \end{equation}
% Under the Gaussian distribution, the $2\hat{\sigma}_i$ interval around the mean value corresponds to $\text{IC}^*=0.9545$, which means the percent of ground-truth values falling within $2\hat{\sigma}_i$ is ideally to be $95.45\%$ for well-calibrated models\cite{pearce2018high}.
% The closer the empirical value to $\text{IC}^*$, the better calibrated the model is.
% Therefore, we define a simpler measure, the $2\hat{\sigma}$ coverage error (ICE), which measures the absolute difference to the ground value $\text{IC}^*$ as:
% \begin{equation}
% \text{ICE} = | \text{IC} - 0.9545 |.
% \end{equation}


% \begin{table}[htbp]
% \begin{center}
%   \caption{5-min ahead prediction metrics for Bitfinex markets.
%   Out of sample performance of 5-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models.}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & MAPE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & ICE $\downarrow$ & IW $\downarrow$ & IW^* $\downarrow$ \\
%     \hline
%   AR-GARCH & 63.952 & 38.229 & 3.3568 & 5.4866 & 0.5268 & 0.0123 & 284.5985 & 68.7842\\
%   AR-GJR-GARCH & 63.78 & 38.838 & 3.7149 & 5.4799 & 0.5306 & 0.0121 & 282.8429 & 68.3496\\
%   AR-TARCH  & 63.696 & 38.523 & 3.585 & 5.4464 & 0.5319 & 0.0127 & 272.1489 & 65.805\\
%   \hline
%   ARX-GARCH  & 63.677 & 38.086 & 3.3441 & 5.482 & 0.531 & 0.012 & 282.9337 & 68.3612\\
%   ARX-GJR-GARCH & 63.597 & 37.208 & 3.2239 & 5.4788 & 0.532 & 0.0109 & 285.3228 & 68.8656\\
% %   ARX-TARCH & 63.727 & 37.139 & 5.4489 & 0.5296 & 0.966& 277.255\\
%     \hline
%   Gradient boosting  & 62.529 & 37.768 & NA & NA & 0.562& NA & NA & NA\\
%   \hline
%   Mixture ensemble &  63.68 & 33.72 & NA & 4.82 & 0.55 & 0.002 & 184.54 & \\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:5minNotNorm}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{5-min ahead prediction metrics for Bitfinex markets \textbf{log volume}.
%   Out of sample performance of 5-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models.
% %   The order $p=10$ for AR-GARCH family was set by using partial auto-correlation function. 
% }
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & MAPE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & ICE & IW $\downarrow$ & IW* $\downarrow$ \\
% \hline
% AR-GARCH     & 66.871 & 33.849 & 1.7273 & 4.6402 & 0.5179 & 0.0115 & 4.6095 & 88.2074\\
% AR-GJR-GARCH & 66.622 & 33.885 & 1.7802 & 4.6397 & 0.52 & 0.0091 & 4.7088 & 88.9369\\
% AR-TARCH     & 66.581 & 33.869 & 1.767 & 4.6389 & 0.52 & 0.0113 & 4.6717 & 82.8026\\
% ARMA-GARCH   & 67.69 & 33.869 & 1.6503 & 4.643 & 0.5118 & 0.011 & 4.5728 & 82.8458\\
% \hline
% ARX-GARCH     & 66.838 & 33.682 & 1.7256 & 4.638 & 0.5213 & 0.0134 & 4.5605 & 84.4472\\
% ARX-GJR-GARCH & 66.673 & 33.721 & 1.7655 & 4.6361 & 0.5229 & 0.0062 & 4.7139 & 90.431\\
% ARX-TARCH     & 66.635 & 33.731 & 1.764 & 4.6357 & 0.523 & 0.0102 & 4.6569 & 82.2032\\
% \hline
% GBM           & 65.027 & 32.683 & NA    & NA     & 0.5661 & NA      & NA & NA \\
% GBM-GARCH     & 65.027 & 32.683 & NA    & 4.6431 & 0.5661 & 0.0266  & 4.4458 & 73.3243 \\
% TME           & 63.794 & 33.604 & 2.087 & 4.649  &        & 0.0215  & 4.196 & 74.212\\
% \hline
% \end{tabular}
% \end{center}
% \label{tab:5minNotNorm}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{5-min ahead prediction metrics for Bitstamp markets.
%   Out of sample performance of 5-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models. }
%   \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ &  MAPE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & ICE $\downarrow$ & IW $\downarrow$  & IW^* $\downarrow$\\
%     \hline
%     AR-GARCH & 38.118 & 17.089 & 3.9858 & 4.9026 & 0.4799 & 0.0223 & 158.4956 & 38.7065\\
%     AR-GJR-GARCH & 38.051 & 17.328 & 4.4906 & 4.8952 & 0.4819 & 0.0228 & 162.6316 & 39.7347\\
% %    AR-TARCH & 38.101 & 17.219 & 4.8802 &  0.4808 &  0.976 & 151.185\\
%     \hline
%     ARX-GARCH & 39.13 & 20.356 & 6.284 & 4.931 & 0.4534 & 0.0237 & 157.9586 & 38.6281\\
%     ARX-GJR-GARCH & 39.131 & 20.324 & 6.2426 & 4.9251 & 0.453 & 0.0234 & 158.1599 & 38.6656\\
% %    ARX-TARCH & 39.159 & 20.087 & 4.9333 &  0.4456 &  0.977 & 156.047\\
%     \hline
%     Gradient boosting & 37.764 & 15.966 & NA & NA & 0.5177& NA & NA & NA\\
%     \hline
%     Mixture ensemble &  38.90 &  15.54 & NA& 3.89 & 0.51 & 0.005 & 91.69 &  \\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:5minNotNorm}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{5-min ahead prediction metrics for Bitstamp markets for \textbf{log volume}.
%   Out of sample performance of 5-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models. }
%   \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ &  MAPE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & ICE & IW $\downarrow$ & IW* $\downarrow$ \\
%     \hline
%   AR-GARCH & 40.332 & 15.605 & 2.541 & 3.7863 & 0.446 & 0.0127 & 5.0069 & 53.6786\\
%   AR-GJR-GARCH  & 40.229 & 15.607 & 2.5404 & 3.7809 & 0.4471 & 0.0079 & 5.0753 & 56.6911\\
%   AR-TARCH    & 40.248 & 15.605 & 2.5382 & 3.7818 & 0.4469 & 0.0119 & 4.9955 & 50.0935\\
%   ARMA-GARCH & 40.496 & 14.93 & 1.7828 & 3.7337 & 0.4477 & 0.0159 & 4.7047 & 35.9107\\
%   \hline
%   ARX-GARCH    & 40.173 & 15.401 & 2.4351 & 3.7754 & 0.4195 & 0.0167 & 4.9289 & 49.6648\\
%   ARX-GJR-GARCH & 40.117 & 15.368 & 2.3979 & 3.7733 & 0.4298 & 0.015 & 4.9661 & 46.3959\\
%   ARX-TARCH    & 40.09 & 15.386 & 2.4265 & 3.7705 & 0.4293 & 0.0139 & 4.9408 & 47.0626\\
%   \hline
%   GBM & 39.156  & 14.594 & NA    & NA    & 0.5261 & NA     & NA & NA \\
%   TME & 39.853  & 14.857 & 2.173 & 3.760 &        & 0.0210 & 4.273  & 43.254 \\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:5minNotNorm}
% \end{table}


%\begin{table*}[htbp]
%\begin{center}
%  \caption{5-min ahead prediction metrics for both markets conditional to the quartile of the target volume in the period of June 2018 - November 2018. }
%  \begin{tabular}{|c|c|c|c|c|}
%  \hline
%  \textbf{BITFINEX MARKET} & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4 \\ 
%  \hline 
%  AR-GARCH & 25.4712 & 32.5289 & 41.3908 & 116.2046\\
%  ARX-GARCH &  29.0931 & 31.2223 & 34.6301 & 114.9813\\
%  Gradient Boosting & 30.9203 & 29.4742 & 28.4582 & 112.6362 \\
%  Mixture ensemble & 22.82 & 21.06 & 25.74 & 120.93 \\
%  \hline
%  & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4 \\ 
%  \hline
%  AR-GARCH & 18.7562 & 21.1582 & 27.2724 & 80.4797\\
  %AR-GARCH(p=1, o=1, q=1) & 18.7561 & 21.1581 & 27.2723 & 80.4797\\
  %AR-GARCH(p=1, o=1, q=1, power=1.0) & 18.1028 & 20.3622 & 26.5371 & 80.5414 \\
%  ARX-GARCH & 24.9695 & 23.1059 & 22.5028 & 77.9657\\
  %ARX-GARCH(p=1, o=1, q=1) & 25.3159 & 25.2036 & 25.2864 & 75.7795\\
  %ARX-GARCH(p=1, o=1, q=1, power=1.0) & 22.804 & 22.518 & 24.1018 & 78.0864\\
 % Gradient Boosting & 28.0851 & 24.4661 & 20.2829 & 74.4320 \\
 % Mixture ensemble & 20.90 & 15.14 & 16.94 & 84.49 \\
 % \hline \hline
 % \textbf{BITSTAMP MARKET} & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4 \\ 
 % \hline
 % AR-GARCH & 11.5399 & 14.5152 & 17.962 & 73.2483\\
 % ARX-GARCH & 18.9325 & 19.0446 & 18.1409 & 71.2284\\
 % Gradient Boosting & 11.4270 & 11.0809 & 10.5455 & 72.6233\\
 % Mixture ensemble & 11.73 & 11.34 & 11.10 & 74.87 \\
 % \hline
 % & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4 \\ 
 % \hline
 % AR-GARCH & 7.6147 & 8.7595 & 10.5267 & 40.2782 \\
  %AR-GARCH(p=1, o=1, q=1) & 7.8134 & 9.0425 & 10.7508 & 40.3151 \\
  %AR-GARCH(p=1, o=1, q=1, power=1.0) & 11.1784 & 13.9888 & 17.0466 & 73.4127\\
 % ARX-GARCH & 17.3215 & 15.8453 & 12.4302 & 35.6983 \\
  %ARX-GARCH(p=1, o=1, q=1) & 14.3531 & 14.9853 & 13.8183 & 37.2452\\
  %ARX-GARCH(p=1, o=1, q=1, power=1.0) & 13.0051 & 13.4347 & 12.197 & 37.5768 \\
 % Gradient Boosting & 10.0851 & 8.7940 & 7.1503 & 37.4343 \\
 % Mixture ensemble & 11.15 & 8.55 & 5.77 & 39.13 \\
 % \hline
%\end{tabular}
%\end{center}
%\label{tab:5minQ1Q4}
%\end{table*}


%In the Appendix (see Table 7-10), we analyze the effects of learning volume in the logarithmic domain for predicting "raw" volumes in the linear domain. We observe that RMSE gets worse, but it can in reducing MAE error. One has to be careful when comparing uncertainty in log and linear domain. Additionally, in the log domain, there are more numerical problems, that have to be addressed due to the presence of zero-values on certain time-scales. 

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.98\textwidth]{figures/m1_t5_src.pdf}
% \caption{Data source contribution for a time series sample of 5 min trading volume in Bitfinex. The contributions are obtained with the temporal mixture ensemble.
% }
% \label{fig:market1_5min_mixing}
% \end{figure}

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.98\textwidth]{figures/m2_t5_src.pdf}
% \caption{Data source contribution for a time series sample of 5 min trading volume in Bitstamp. The contributions are obtained with the temporal mixture ensemble.
% }
% \label{fig:market2_5min_mixing}
% \end{figure}


%  \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.98\textwidth]{figures/m1_t1_src.pdf}
% \caption{Data source contribution for a time series sample of 1 min trading volume in Bitfinex. The contributions are obtained with the temporal mixture ensemble model.
% }
% \label{fig:market1_1min_mixing}
% \end{figure}


% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.98\textwidth]{figures/m2_t1_src.pdf}
% \caption{Data source contribution for a time series sample of 5 min trading volume in Bitstamp. The contributions are obtained with the temporal mixture ensemble model.
% }
% \label{fig:market2_1min_mixing}
% \end{figure}

% \begin{table*}[htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics for both markets conditional to the quartile of the target volume in the period of June 2018 - November 2018. }
%   \begin{tabular}{|c|c|c|c|c|}
%   \hline
%   \textbf{BITFINEX MARKET}  & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4\\ 
%   \hline
%   AR-GARCH & 7.3131 & 9.163 & 10.3165 & 37.0707\\
%   ARX-GARCH& 7.0584 & 9.0724 & 10.1451 & 37.2288\\
%   Gradient Boosting & 5.2867 & 5.9321 & 6.0074 & 38.7101\\
%   Mixture ensemble& 6.59 & 7.56 & 8.086 & 37.86 \\
%   \hline
%   & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4  \\ 
%   \hline
%   AR-GARCH & 5.8234 & 6.3874 & 5.9997 & 21.5342\\
%   ARX-GARCH& 5.2314 & 5.9161 & 5.8702 & 21.7944\\
%   Gradient Boosting & 4.6802 & 4.78 & 3.8955 & 22.1228\\
%   Mixture ensemble& 6.07 & 6.16 & 4.84 & 21.70 \\
%   \hline \hline
%   \textbf{BITSTAMP MARKET}  & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4   \\ 
%   \hline
%   AR-GARCH & 3.3807 & 3.9941 & 4.376 & 21.3262\\
%   ARX-GARCH& 3.7292 & 4.3312 & 4.6574 & 21.2603\\
%   Gradient Boosting & 2.0817 & 2.2466 & 2.1172 & 22.0518\\
%   Mixture ensemble& 2.71 & 2.89 & 2.64 & 22.19 \\
%   \hline
%   & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4\\ 
%   \hline
%   AR-GARCH & 2.4622 & 2.5202 & 2.2675 & 9.7414\\
%   ARX-GARCH & 2.8769 & 2.9354 & 2.6175 & 9.5851\\
%   Gradient Boosting & 1.7587 & 1.7614 & 1.3628 & 10.0345\\
%   Mixture ensemble& 2.46 & 2.40 & 1.55 & 9.90 \\
%   \hline
% \end{tabular}
% \end{center}
% \label{tab:1minQ1Q4}
% \end{table*}

% \begin{table*}[htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics for both markets for \textbf{log volume} conditional to the quartile of the target volume in the period of June 2018 - November 2018. }
%   \begin{tabular}{|c|c|c|c|c|}
%   \hline
%   \textbf{BITFINEX MARKET}  & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4\\ 
%   \hline
%  AR-GARCH & 2.3579 & 3.1555 & 4.5016 & 42.2563\\
%  AR-GJR-GARCH & 2.3179 & 3.075 & 4.3936 & 42.3838\\
%  AR-TARCH & 2.3137 & 3.0921 & 4.4501 & 42.3315\\
%  ARMA-GARCH & 2.0444 & 2.8593 & 4.216 & 42.9823\\
%  ARX-GARCH & 2.2627 & 2.9996 & 4.371 & 42.4405\\
%  GBM & 
% 2.0956 & 2.7643 & 4.2074 & 41.7473\\
%   \hline
%   & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4  \\ 
%   \hline
% AR-GARCH& 1.4624 & 1.8402 & 3.2237 & 25.9867\\
% AR-GJR-GARCH & 1.4492 & 1.8052 & 3.179 & 26.1027\\
% AR-TARCH & 1.4301 & 1.8018 & 3.2082 & 26.0757\\
% ARMA-GARCH & 1.2863 & 1.6747 & 3.1537 & 26.6452\\
% ARX-GARCH & 1.4282 & 1.7665 & 3.1583 & 26.1776\\
% GBM & 
% 1.5122 & 1.5935 & 3.0119 & 25.728\\
%   \hline \hline
%   \textbf{BITSTAMP MARKET}  & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4   \\ 
%   \hline
%  AR-GARCH & 1.2215 & 1.319 & 1.681 & 24.3689\\
%  AR-GJR-GARCH & 1.2283 & 1.3336 & 1.702 & 24.3276\\
%  AR-TARCH & 1.2259 & 1.3332 & 1.7066 & 24.3214\\
%  ARMA-GARCH & 0.8625 & 1.0347 & 1.7208 & 24.6277\\
%  ARX-GARCH & 1.123 & 1.3641 & 1.809 & 24.2962\\
%  GBM & 
% 0.8799 & 1.0328 & 1.6891 & 23.3448\\
%   \hline
%   & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4\\ 
%   AR-GARCH & 0.7751 & 0.7951 & 1.3045 & 11.7734\\
%   AR-GJR-GARCH & 0.772 & 0.7974 & 1.3166 & 11.7487\\
%   AR-TARCH & 0.7678 & 0.7947 & 1.3199 & 11.7492\\
%   ARMA-GARCH & 0.5305 & 0.6007 & 1.3578 & 12.035\\
%   ARX-GARCH & 0.7374 & 0.7555 & 1.2986 & 11.7957\\
%   GBM & 
% 0.5935 & 0.5823 & 1.2957 & 11.5491\\
%   \hline
%   \hline
% \end{tabular}
% \end{center}
% \label{tab:1minQ1Q4}
% \end{table*}



% \iffalse
% \begin{table}[htbp]
% \begin{center}
%   \caption{1-min Ahead Prediction for Market 1 that corresponds to the period of June 2018 - October 2018. in logarithmic learning setting $\hat{v_t}=\ln(v_t)$. RMSE, MAE and CORR are evaluated on "raw" linear volumes $v_t$, by using exponent function on predictions $exp(\hat{v}_t)$. Likelihood was calculated for log-normal distribution (NNLL). IC and IW were calculated over $\hat{v_t}=\ln(v_t)$ values with two--$\sigma$ upper and lower level under the Gaussian assumption over $\ln(v_t)$ domain. Note, that one should be careful not to directly compare results in logarithmic and "raw" linear volume domain e.g. likelihood and interval coverage in log and linear domain. NAN* values indicate certain numerical problems due to the presence of zero-volume on certain time-scales. }
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & IC (0.954) & IW $\downarrow$ \\
%     \hline
%     AR-GARCH  & 21.324 & 8.139 & 2.666
%     & 0.4404 & 0.944 & 7.83\\%
%     AR-GJR-GARCH & 21.378 & 8.144 & 2.661  & 0.4414 &  0.947 & 7.86\\ %
%     AR-TARCH & 21.354 & 8.138 & 2.6583  & 0.4413 & 0.947 & 7.802\\%
%     \hline
%     ARX-GARCH & NAN & NAN & NAN & NAN & NAN & NAN\\
%     ARX-GJR-GARCH & NAN & NAN & NAN & NAN & NAN & NAN\\
%     ARX-TARCH & NAN & NAN & NAN & NAN & NAN & NAN\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1minLog_m1}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{1-min Ahead Prediction for Market 2 that corresponds to the period of June 2018 - October 2018. in logarithmic learning setting $\hat{v_t}=\ln(v_t)$. RMSE, MAE and CORR are evaluated on "raw" linear volumes $v_t$, by using exponent function on predictions $exp(\hat{v}_t)$. Likelihood was calculated for log-normal distribution (NNLL). IC and IW were calculated over $\hat{v_t}=\ln(v_t)$ values with two--$\sigma$ upper and lower level under the Gaussian assumption over $\ln(v_t)$ domain. Note, that one should be careful not to directly compare results in logarithmic and "raw" linear volume domain e.g. likelihood and interval coverage in log and linear domain. NAN* values indicate certain numerical problems due to the presence of zero-volume on certain time-scales. }
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & IC (0.954) & IW $\downarrow$ \\
%     \hline
%     AR-GARCH  & 12.201 & 3.607 & 1.7201
%     & 0.4234 &  0.943 & 8.655\\ 
%     AR-GJR-GARCH & 12.21 & 3.608 & 1.7173 & 0.4244 &  0.947 & 8.724\\
%     AR-TARCH & 12.25 & 3.615 & 1.7276  & 0.4261 & 0.932 & 8.178\\
%     \hline
%     ARX-GARCH & 12.19 & 3.603 & 1.7198 & 0.4147 & 0.943 & 8.654\\
%     ARX-GJR-GARCH & NAN & NAN & NAN & NAN & NAN & NAN\\
%     ARX-TARCH & NAN & NAN & NAN & NAN & NAN & NAN\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1minLog_m1}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{5-min Ahead Prediction for Market 1 that corresponds to the period of June 2018 - October 2018. in logarithmic learning setting $\hat{v_t}=\ln(v_t)$. RMSE, MAE and CORR are evaluated on "raw" linear volumes $v_t$, by using exponent function on predictions $exp(\hat{v}_t)$. Likelihood was calculated for log-normal distribution (NNLL). IC and IW were calculated over $\hat{v_t}=\ln(v_t)$ values with two--$\sigma$ upper and lower level under the Gaussian assumption over $\ln(v_t)$ domain. Note, that one should be careful not to directly compare results in logarithmic and "raw" linear volume domain e.g. likelihood and interval coverage in log and linear domain. }
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & IC (0.954) & IW $\downarrow$ \\
%     \hline
%     AR-GARCH  & 66.909 & 33.838 & 4.6401 & 0.5187 & 0.943 & 4.604\\ 
%     AR-GJR-GARCH & 67.032 & 33.823 & 4.6331 & 0.5195 & 0.95 & 4.663\\
%     AR-TARCH & 67.0 & 33.808 & 4.632 & 0.5194 & 0.949 & 4.63\\
%     \hline
%     ARX-GARCH  & 66.852 & 33.688 & 4.6372 & 0.5219 & 0.943 & 4.591\\
%     ARX-GJR-GARCH & 67.037 & 33.687 & 4.6304 & 0.5228 &  0.949 & 4.654\\
%     ARX-TARCH & NAN & NAN & NAN & NAN & NAN & NAN\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:5minLog}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{5-min Ahead Prediction for Market 2 that corresponds to the period of June 2018 - October 2018. in logarithmic learning setting $\hat{v_t}=\ln(v_t)$. RMSE, MAE and CORR are evaluated on "raw" linear volumes $v_t$, by using exponent function on predictions $exp(\hat{v}_t)$. Likelihood was calculated for log-normal distribution (NNLL). IC and IW were calculated over $\hat{v_t}=\ln(v_t)$ values with two--$\sigma$ upper and lower level under the Gaussian assumption over $\ln(v_t)$ domain. Note, that one should be careful not to directly compare results in logarithmic and "raw" linear volume domain e.g. likelihood and interval coverage in log and linear domain. }
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & IC (0.954) & IW $\downarrow$ \\
%     \hline
%     AR-GARCH  & 40.041 & 14.932 & 3.7338 & 0.464 & 0.939 & 4.737\\ %
%     AR-GJR-GARCH & 40.089 & 14.922 & 3.728  & 0.4652 &  0.944 & 4.853\\ %
%     AR-TARCH & 40.075 & 14.918 & 3.7271  & 0.4654 &  0.942 & 4.743\\%
%     \hline
%     ARX-GARCH  & 39.86 & 14.91 & 3.7346 & 0.4645 &  0.939 & 4.735\\%
%     ARX-GJR-GARCH & NAN & NAN & NAN & NAN & NAN & NAN\\%
%     ARX-TARCH & NAN & NAN & NAN & NAN & NAN & NAN\\%
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:5minLog_m2}
% \end{table}

% \begin{figure*}[!htb]
% \begin{center}
% \piclabC{intraday_avg_std_volume_2019_large_sample_1min.pdf}{}
% \piclabC{volume_min_distr_6months_2019.pdf}{}
% \piclabC{intraday_avg_std_volume_2019_large_sample_5min.pdf}{}
% \end{center}
% \caption{ \textbf{First row} The intraday average 1-min volume plus 1 std over period of 6 months in 2019.
% \textbf{Second row} The distribution of  1-min volume over period of 6 months in 2019.
% \textbf{Third row} The intraday average 5-min  volume plus 1 std over period of 6 months in 2019.
% }
% \label{fig:volume_statistics2}
% \end{figure*}


% \begin{table}[htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics for Bitstamp markets.
%   Out of sample performance of 1-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models. 
%   }
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & ICE $\downarrow$& IW $\downarrow$\\
%     \hline
%     AR-GARCH & 11.196 & 4.248 & 3.5866 & 0.4774 & 0.023 & 40.115\\
%     AR-GJR-GARCH & 11.193 & 4.243 & 3.5841 &  0.4762 & 0.023 & 42.34\\
%  %   AR-TARCH & 11.24 & 4.314 & 3.5438 & 0.4762 & 0.978 & 39.341\\
%     \hline
%     ARX-GARCH & 11.252 & 4.504 & 3.5895 &  0.4701  &  0.023 & 39.794\\
%     ARX-GJR-GARCH & 11.21 & 4.188 & 3.5862 & 0.4739 & 0.023 & 41.598\\
% %    ARX-TARCH*& NAN & NAN & NAN & NAN & NAN & NAN\\
%     \hline
%     Gradient boosting & 11.182 & 3.73 & NA & 0.5317& NA & NA\\
%     \hline
%     Mixture ensemble &  11.38 &  4.058 & 2.03 & 0.49 & 0.004 & 27.67 \\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1minNotNorm}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics for Bitstamp markets for \textbf{log volume}.
%   Out of sample performance of 1-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models. 
%   }
%   \begin{tabular}{|c|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & RelMAE $\downarrow$ & CORR $\uparrow$ & IC & IW $\downarrow$\\
%     \hline
% AR-GARCH & 12.246 & 3.662 & 1.7434 & 38.6133 & 0.4402 & 0.941 & 8.89\\
% AR-GJR-GARCH & 12.227 & 3.659 & 1.7417 & 38.3774 & 0.4413 & 0.941 & 8.875\\
% AR-TARCH & 12.224 & 3.658 & 1.7453 & 38.1636 & 0.4416 & 0.936 & 8.622\\
% ARMA-GARCH & 12.363 & 3.631 & 1.7111 & 26.4304 & 0.4031 & 0.945 & 8.542\\
% \hline
% ARX-GARCH & 12.216 & 3.647 & 1.7415 & 38.8222 & 0.3714 & 0.934 & 8.545\\
% ARX-GJR-GARCH & 12.211 & 3.642 & 1.7349 & 38.2388 & 0.3884 & 0.941 & 8.764\\
% ARX-TARCH & 12.203 & 3.641 & 1.7371 & 38.5076 & 0.3884 & 0.938 & 8.616\\
% \hline
% GBM & 11.723 & 3.505 & NA & NA & 0.5211& NA & NA\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1minNotNorm}
% \end{table}


% \begin{table}[htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics for Bitfinex markets.
%   Out of sample performance of 1-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models.
%   }
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & CORR $\uparrow$ & ICE $\downarrow$ & IW $\downarrow$\\
%     \hline
%     AR-GARCH & 20.113 & 9.936 & 4.2542 & 0.447 & 0.016 & 86.523 \\
%     AR-GJR-GARCH & 20.086 & 9.976 & 4.2522 & 0.4471 & 0.016 & 86.366\\
% %    AR-TARCH & 20.137 & 9.929 & 4.2178 & 0.4466  & 0.97 & 82.249\\
%     \hline
%     ARX-GARCH & 20.132 & 9.703 & 4.2445 &  0.4451 & 0.015 & 85.423\\
%     ARX-GJR-GARCH & 20.103 & 9.867 & 4.2494 & 0.4453  & 0.016 & 86.603\\
% %    ARX-TARCH*& NAN & NAN & NAN & NAN & NAN & NAN\\
%     \hline
%     Gradient boosting & 19.985 & 8.87 & NA & 0.483& NA & NA\\
%     \hline
%     Mixture ensemble & 20.00 & 9.42 & 2.90 & 0.46 & 0.001 & 61.89\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1minNotNorm}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics for Bitfinex markets for \textbf{log volume}.
%   Out of sample performance of 1-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models.
%   }
%   \begin{tabular}{|c|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & RelMAE $\downarrow$ & CORR $\uparrow$ & IC & IW $\downarrow$\\
%     \hline
%   AR-GARCH & 21.339 & 8.129 & 2.6631 & 89.6834 & 0.4388 & 0.944 & 7.819\\
%   AR-GJR-GARCH & 21.393 & 8.134 & 2.6581 & 88.9665 & 0.44 & 0.947 & 7.843\\
%   AR-TARCH & 21.37 & 8.129 & 2.6554 & 86.208 & 0.44 & 0.947 & 7.79\\
%   ARMA-GARCH & 21.665 & 8.19 & 2.6595 & 89.6697 & 0.4271 & 0.945 & 7.756\\
%   \hline
%   ARX-GARCH & 21.416 & 8.133 & 2.6631 & 87.0867 & 0.4344 & 0.941 & 7.686\\
%   ARX-GJR-GARCH & 21.48 & 8.143 & 2.6574 & 88.2053 & 0.4385 & 0.945 & 7.775\\
%   ARX-TARCH & 21.431 & 8.134 & 2.6546 & 86.2742 & 0.4384 & 0.946 & 7.765\\
%   \hline
%   GBM & 21.05 & 7.961 & NA & NA & 0.4741& NA & NA\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1minNotNorm}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics for Bitstamp markets for \textbf{log volume and point and distribution linear evaluation}.
%   Out of sample performance of 1-min ahead predictions for the period of June 2018 - November 2018 (70\% train, 10\% validation and 20\% test). The arrow symbols in the first line indicate the direction of the metrics for better models.
%   }
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ & MAPE $\downarrow$ & NNLL $\downarrow$ & IC & IW $\downarrow$\\
%     \hline
% ARMAX(6,4)-GARCH(1,1) & 39998.9444 & 1304.5381 & 6317.3749 & 1.7282 & 0.9448 & 1383.7328\\
% ARMA(6,4)-GARCH(1,1) & 842.0767 & 36.6622 & 378.4516 & 1.7292 & 0.945 & 174.515\\
%  GBM  & 11.7334 & 3.5058 & 3.2612 & NA & NA & NA\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1minNotNorm}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{10-min ahead prediction metrics for Bitstamp market.
%   The arrow symbols in the first line indicate the direction of the metrics for better models.}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|}
%     \hline
%     MODEL & RMSE $\downarrow$ & MAE $\downarrow$ &  MAPE $\downarrow$ & NNLL $\downarrow$ & IC & IW $\downarrow$ \\
%     \hline
% ARMA(2,3)-GARCH(1,1)  & 66.5021 & 32.1228 & 1.8836 & 4.4534 & 0.9407 & 190.3937\\
% ARMAX(2,3)-GARCH(1,1) & 73.2577 & 33.4053 & 1.8441 & 4.479 & 0.9383 & 197.1746\\
% GBM & 67.2064 & 27.4485 & 1.0351 & NA & NA & NA\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:5minNotNorm}
% \end{table}


\subsection{Baseline details} \label{appB}


\subsubsection{Econometric benchmarks}

As mentioned, our benchmarks belong to the AR-GARCH class with external regressors. More specifically, the volume process $y_t$ is modelled with the following autoregressive process (AR(p)) with external regressors:\\
\begin{equation}
y_t = \mu + \sum_{i=1}^p \phi_i y_{t-i} +  \sum_{s=1}^{S} \sum_{j=1}^{d_s}\psi_{s,j} \mathbf{x}_{s,t-1}(j)  + \epsilon_t,
\end{equation}
where $\mathbf{x}_{s,t-1}(j)$ denotes the $j$-th feature from external feature vector $\mathbf{x}_{s,t-1}$ at time\footnote{Note, that we have also evaluated all ARX-GARCH models by using autoregressive external features $\{ \mathbf{x}_{s,t-i}(j) \}_{i=1}^p$ terms, but results were not better and training time and convergence become problematic.} $t-1$ from source $s$. The total number of sources $S=4$, which includes transactions and limit order book data of the two markets.  
Since volume exhibits time clustering, we assume that the residuals $\epsilon_t$ are modelled by a GARCH process \cite{brownlees2010intra, satish2014predicting, chen2016forecasting}:
\begin{equation}
\epsilon_t = \sigma_t e_t~~~~~~~ e_t \sim \mathcal{N}(0,1)
\end{equation}
 \begin{equation}
\sigma_t^{\lambda} = \omega + \alpha\epsilon_{t-1}^{\lambda} + \gamma |\epsilon_{t-1}|^{\lambda}\mathbbm{1}_{[\epsilon_{t-1}<0]} + \beta\sigma_{t-1}^{\lambda}
 \end{equation}

For $\lambda=2$, $\gamma=0$, we get standard GARCH(1,1) model \cite{GARCH}. In case of $\lambda=2$, $\gamma=1$, we get GJR-GARCH model \cite{GJR-GARCH}, that captures asymmetry in positive and negative shocks\footnote{We also tested the case of $\lambda=1$, $\gamma=1$ corresponding to the Threshold heteroskedastic models \cite{TARCH}, but the model displays sometimes convergence problems, thus we decided not to present it. Anyhow the forecasting ability of this model is comparable to that of the other GARCH models.}.

\subsubsection{Machine learning benchmark}

We take the gradient boosting machine \cite{friedman2001greedy} as a machine learning baseline. 
Gradient boosting approximates the volume $\hat{y_t}=F(\mathbf{x}_{<t})$ with a function that has the following additive expansion (similar to other functional approximation methods like radial basis functions, neural networks, wavelets, etc.):
\begin{equation}
\hat{y_t}=F(\mathbf{x}_{<t})=\sum_{m=0}^M \beta_m h(\mathbf{x}_{<t};\mathbf{a}_m),
\end{equation}
where $\mathbf{x}_{<t}$ denotes the feature vector, that is constructed as a concatenation from different sources\footnote{Note, that we have omitted the transpose operators in the next line, as the concatenation is simple operation and to avoid confusion with index of time.} $\mathbf{x}_{t}=(\mathbf{x}_{s=1,<t},\mathbf{x}_{s=2,<t},\mathbf{x}_{s=3,<t},\mathbf{x}_{s=4,<t})$ .
 
The functions $h(\mathbf{x}_{<t};\mathbf{a}_m)$ are also called "base learners" and in our case they are regression trees with parameters $\mathbf{a}_m$ and $\beta_m$ is a simple scalar. 

Each base learner $h(\mathbf{x}_{<t};\mathbf{a}_m)$ partitions the feature space $\mathbf{x}_{<t} \in \mathbf{X}$
into $L$-disjoint regions $\{R_{l,m}\}_1^L$ and predicts a separate constant value in each:
\begin{equation}
h(\mathbf{x}_{t};\{R_{l,m}\}_1^L)= \sum_{l=1}^L \bar{y}_{l,m} \mathbf{1}(\mathbf{x}_{<t} \in R_{l,m}),
\end{equation}
where $\bar{y}_{l,m}$ is inferred during the learning phase along with the expansion coefficients $\{ \beta_m \}$ and the parameters of regression trees $\mathbf{a}_m$. Learning procedure starts by defining the loss function $\Psi(y_t,F(\mathbf{x}_{<t}))$ e.g. squared loss $\sum_t (y_t-F(\mathbf{x}_{<t}))^2$ and initial regression tree $F_0(\mathbf{x}_{<t})$. Then, for each $m=1,...,M$, we solve the optimization problem:
\begin{equation}
(\beta_m, \mathbf{a}_m) = \argmin_{\beta, \mathbf{a}} \sum_{t=1}^{T} \Psi(y_t, F_{m-1}(\mathbf{x}_{<t}) + \beta h(\mathbf{x}_{<t};\mathbf{a}) )
\end{equation}
and
\begin{equation}
F_{m}(\mathbf{x}_{<t})= F_{m-1}(\mathbf{x}_{<t}) + \beta_m h(\mathbf{x}_{<t};\mathbf{a}_m).
\end{equation}
See Appendix for more details. Furthermore, note that different variants of tree boosting have been empirically proven to be state-of-the-art methods in predictive tasks across different machine learning challenges \cite{nielsen2016tree,taieb2014gradient} and more recently in finance\cite{zhou2015evolution, sun2018novel}.


For a given training sample $\{ y_t, \mathbf{x}_<t \}_{t=1}^T$, 
our goal is to find a function $F^*(\mathbf{x})$ such that the expected value of loss function $\Psi(y, F(\mathbf{x}))$ is minimized over the joint distribution of $\{ y, \mathbf{x} \}$
\begin{equation}
F^*(\mathbf{x}) = \argmin_{F(x)} \mathbb{E}_{y, \mathbf{x}} \Psi(y, F(\mathbf{x})).
\end{equation}
Under the additive expansion $F(\mathbf{x})=\sum_{m=0}^M \beta_m h(\mathbf{x};\mathbf{a}_m)$ with parameterized functions $h(\mathbf{x};\mathbf{a}_m)$, we proceed with the minimization of data estimate of expected loss \cite{friedman2001greedy}:
\begin{equation}
\{\beta_m, \mathbf{a}_m\}_1^M = \argmin_{\beta_m^{'}, \mathbf{a}_m^{'}} \sum_{t=1}^{T} \Psi(y_t, \sum_{m=0}^M \beta^{\prime}_m h(\mathbf{x}_{<t};\mathbf{a}^{\prime}_{m}) ).
\end{equation}
However, for practical purposes first we make the initial guess\\ $F_0(\mathbf{x})=\argmin_{c} \sum_{t=1}^T \Psi(y_t, c)$ and then parameters are jointly fit in a forward incremental way $m=1,...,M$:
\begin{equation}
(\beta_m, \mathbf{a}_m) = \argmin_{\beta, \mathbf{a}} \sum_{t=1}^{T} \Psi(y_t, F_{m-1}(\mathbf{x}_{<t}) + \beta h(\mathbf{x}_{t};\mathbf{a}) )
\end{equation}
and
\begin{equation}
F_{m}(\mathbf{x}_{<t})= F_{m-1}(\mathbf{x}_{<t}) + \beta_m h(\mathbf{x}_{<t};\mathbf{a}_m).
\end{equation}
First, the function $h(\mathbf{x}_{<t};\mathbf{a})$ is fit by least-squares to the pseudo-residuals $\widetilde{y}_{t,m}$
\begin{equation}
\mathbf{a}_m = \argmin_{\mathbf{a}, \rho} \sum_{t=1}^T [ \widetilde{y}_{t,m} - \rho h(\mathbf{x}_{<t};\mathbf{a}) ]^2,
\end{equation}
which for squared loss $\Psi(y_t, F(\mathbf{x}_{<t}))=\frac{1}{2}(y_t- F(x))^2$ at stage $m$ is a residual $\widetilde{y}_{t,m}=(y_t-F_{m-1}(\mathbf{x}_{<t}))$. For general loss $\Psi$, we have
\begin{equation}
\label{eq:pseudo-residual}
\widetilde{y}_{t,m}=-\left[ \frac{\partial\Psi(y_t, F(\mathbf{x}_{<t}))}{\partial F(\mathbf{x}_{<t})} \right]_{F(\mathbf{x})=F_{m-1}(\mathbf{x})}.
\end{equation}
Now, we just find the coefficient $\beta_m$ for the expansion as
\begin{equation}
    \beta_m = \argmin_{\beta} \sum_{t=1}^{T} \psi(y_t, F_{m-1}+\beta h(\mathbf{x}_{<t};\mathbf{a}_m)).
\end{equation}

Each base learner $h(\mathbf{x}_{<t};\mathbf{a}_m)$ partitions the feature space $\mathbf{x}_{<t} \in \mathbf{X}$
into $L$-disjoint regions $\{R_{l,m}\}_1^L$ and predicts a separate constant value in each:
\begin{equation}
h(\mathbf{x}_{<t};\{R_{l,m}\}_1^L)= \sum_{l=1}^L \bar{y}_{l,m} \mathbf{1}(\mathbf{x}_{<t} \in R_{l,m}),
\end{equation}
where $\bar{y}_{l,m}$ is the mean value of pseudo-residual (eq. \ref{eq:pseudo-residual}) in each region $R_{l,m}$
\begin{equation}
\bar{y}_{l,m}=\frac{\sum_{t=1}^T \widetilde{y}_{t,m} \mathbf{1}[\mathbf{x}_{<t} \in R_{l,m}]}{ \sum_{t=1}^T \mathbf{1}[\mathbf{x}_{<t} \in R_{l,m}]}.
\end{equation}
We have used the GBM implementation from Scikit-learn library\cite{scikit-learn} for all our experiments \footnote{Within this library, for hyper-parameters optimization, we take the following regression tree hyper-parameters into the account: "n\_estimators", "max\_features", "min\_samples\_leaf", "max\_depth" and the following learning hyper-parameters: "learning\_rate" and "loss".}.


% \begin{table}[htbp]
% \centering
% \caption{5-min ahead prediction metrics of both markets.
% The arrow symbols indicate the direction of the metrics for better models.}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \textbf{BITFINEX MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$\\
% \hline
% ARMA(3,3)-GARCH(1,1)    & 65.147 & 40.056 & 4.643 & 280.318 \\
% ARMAX(3,3)-GARCH(1,1)   & 81.157 & 40.739 & 4.742 & 279.596 \\
% GBM                     & 65.110 & 32.631 & NA    & NA      \\
% TME                     & 63.756 & 38.867 & 4.644 & 268.118 \\
% \hline
% \hline
% \textbf{BITSTAMP MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$ \\
% \hline
% ARMA(3,2)-GARCH(1,1)  & 38.618  & 17.885 & 3.738  & 118.766\\
% ARMAX(3,2)-GARCH(1,1) & 38.551  & 17.675 & 3.749  & 118.725\\
% GBM                   & 39.174  & 14.613 & NA     & NA \\
% TME                   & 38.238  & 16.935 & 3.736  & 100.923 \\ 
% \hline
% \end{tabular}\label{tab:5min}
% \end{table}

% both considering RMSE and MAE, when Bitfinex volume is in Q1-Q3. 
% For Bitstamp market the results are less clear, but in general machine learning methods work better than the benchmark econometric models. 

% \begin{table*}[htbp]
% \centering
%  \caption{5-min ahead prediction metrics of both markets conditional on the quartile of the target values.}
%  \begin{tabular}{|c|c|c|c|c|}
%  \hline
%  \textbf{BITFINEX MARKET} & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4 \\ 
%  \hline 
% ARMA(3,3)-GARCH(1,1)  & 33.029  & 38.868  & 43.525 & 111.684 \\
% ARMAX(3,3)-GARCH(1,1) & 32.894  & 39.552  & 57.202 & 115.004 \\
% GBM                   & 17.366  & 16.336  & 21.474 & 126.041 \\
% TME                   & 35.557  & 35.863  & 35.991 & 111.430 \\
%  \hline
%  & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4 \\
%  \hline
% ARMAX(3,3)-GARCH(1,1) & 27.593 & 12.378 & 33.105 & 138.259\\
% ARMA(3,3)-GARCH(1,1)  & 26.906 & 28.797 & 29.803 & 74.696 \\
% GBM                   & 14.716 & 11.456 & 16.216 & 88.332 \\
% TME                   & 32.154 & 29.265 & 25.298 & 72.686 \\
%  \hline
%  \hline
%  \textbf{BITSTAMP MARKET} & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4 \\ 
%  \hline
% ARMA(3,2)-GARCH(1,1)  & 14.259 & 15.881 & 16.361 & 72.357 \\
% ARMAX(3,2)-GARCH(1,1) & 13.659 & 15.442 & 16.374 & 72.423 \\
% GBM                   &  6.224 &  6.274 &  8.288 & 77.358 \\
% TME                   & 13.029 & 13.677 & 13.220 & 73.626 \\
%  \hline
%  & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4 \\
%  \hline
% ARMA(3,2)-GARCH(1,1)  & 11.193 & 12.032 & 11.142 & 37.136 \\
% ARMAX(3,2)-GARCH(1,1) & 10.800 & 11.750 & 11.001 & 37.117 \\
% GBM                   &  4.908 &  4.316 &  6.378 & 42.764 \\
% TME                   & 11.454 & 10.737 &  9.262 & 36.608 \\
%  \hline
% \end{tabular}
% \label{tab:5minQ1Q4}
% \end{table*}

% \begin{table*}[!htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics of both markets conditional on the quartile of the target values.}
%   \begin{tabular}{|c|c|c|c|c|}
%   \hline
%   \textbf{BITFINEX MARKET} & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4 \\ 
%   \hline 
% ARMA(5,5)-GARCH(1,1) & 13.713 & 17.3421 & 20.4708 & 39.0995\\
% GBM                   &  &  &  & \\
% TME                   & 6.930 & 8.520 & 8.917 & 37.516 \\
%   \hline
%   & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4 \\
%   \hline
% ARMA(5,5)-GARCH(1,1) & 9.2211 & 11.3326 & 12.7194 & 23.8872\\
% GBM                   &  &  &  & \\
% TME                   & 6.126  & 6.826 & 6.068 & 21.067 \\
%   \hline
%   \hline 
%   \textbf{BITSTAMP MARKET} & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4 \\ 
%   \hline
% ARMA(6,4)-GARCH(1,1)& 762.0322 & 420.2495 & 802.4139 & 1197.9002\\
% ARMAX(2,3)-GARCH(1,1) &  &  &  & \\
% GBM                   &  &  &  & \\
% TME                   & 2.879 & 3.240 & 3.247 & 22.080 \\
%   \hline
%   & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4 \\
%   \hline
% ARMA(6,4)-GARCH(1,1)[LOG-Vol] & 22.5049 & 16.3995 & 36.4212 & 71.3103\\
% GBM                   &  &  &  & \\
% TME                   & 2.511 & 2.622 & 2.113 & 9.572 \\
%   \hline
% \end{tabular}
% \end{center}
% \label{tab:1minQ1Q4}
% \end{table*}



% \begin{table}[!htbp]
% \begin{center}
%   \caption{1-min ahead prediction metrics of both markets. The arrow symbols indicate the direction of the metrics for better models. *Econometric models on Bitstamp market, were having numerical problems.
%   }
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     \textbf{BITFINEX MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$\\
%     \hline
% ARMA(5,5)-GARCH(1,1)  & 24.681 & 14.294 & 2.661  & 126.437 \\
% ARMAX(5,5)-GARCH(1,1) & 24.771 & 14.280 & 2.662  & 126.263 \\
% GBM                   & 21.050 &  7.962 & NA     & NA      \\
% TME                   & 20.053 &  9.207  & 2.645  & 97.106  \\
%     \hline
%     \hline
%     \textbf{BITSTAMP MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$\\
%     \hline
% *ARMAX(6,4)-GARCH(1,1) & 39998.944 & 1304.538 & 1.728  & 1383.733 \\
% *ARMA(6,4)-GARCH(1,1)  & 842.077   & 36.662   & 1.729  & 174.515 \\
% GBM                   & 11.733    & 3.506    &  NA    & NA      \\
% TME                   & 11.344    & 4.203    & 1.711  &  40.768  \\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1min}
% \end{table}




% \begin{table}[!htbp]
% \begin{center}
%   \caption{10-min ahead prediction metrics of both markets.
%   The arrow symbols in the first line indicate the direction of the metrics for better models.}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|}
%     \hline
%     \textbf{BITFINEX MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$ \\
%     \hline
% ARMA(5,4)-GARCH(1,1)  & 111.982  & 70.377 & 5.415 & 442.241\\
% ARMAX(5,4)-GARCH(1,1) & 114.673  & 71.161 & 5.885 & 446.870\\
% GBM                   & 109.994  & 60.832 & NA    & NA\\
% TME                   & 108.500  & 60.762 & 5.363 & 432.233\\
%     \hline
%     \hline
%     \textbf{BITSTAMP MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$ \\
%     \hline
% ARMA(2,3)-GARCH(1,1)  & 66.502 & 32.123 & 4.453  & 190.394 \\
% ARMAX(2,3)-GARCH(1,1) & 73.258 & 33.405 & 4.479  & 197.175 \\
% GBM                   & 67.206 & 27.449 & NA     & NA \\
% TME                   & 67.447 & 32.117 & 4.501  & 172.359 \\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:10min}
% \end{table}


% \begin{table*}[htbp]
% \begin{center}
%   \caption{10-min ahead prediction metrics of both markets conditional on the quartile of the target values.}
%   \begin{tabular}{|c|c|c|c|c|}
%   \hline
%   \textbf{BITFINEX MARKET} & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4 \\ 
%   \hline 
% ARMA(5,4)-GARCH(1,1)  & 58.632 & 65.563 & 67.771 & 194.436 \\
% ARMAX(5,4)-GARCH(1,1) & 59.976 & 66.520 & 69.637 & 192.640 \\
% GBM                   & 38.814 & 36.969 & 43.147 & 208.896 \\
% TME                   & 42.378 & 27.414 & 27.414 & 185.655 \\
%   \hline
%   & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4 \\
%   \hline
% ARMA(5,4)-GARCH(1,1)  & 48.029 & 49.955 & 49.056 & 134.448\\
% ARMAX(5,4)-GARCH(1,1) & 49.147 & 51.246 & 49.997 & 132.500\\
% GBM                   & 34.001 & 27.359 & 32.520 & 149.403\\
% TME                   & 14.079 & 21.544 & 41.553 & 130.538\\
%   \hline
%   \hline
%   \textbf{BITSTAMP MARKET} & RMSE Q1 & RMSE Q2 & RMSE Q3 & RMSE Q4 \\ 
%   \hline
% ARMA(2,3)-GARCH(1,1)  & 25.349 & 28.200 & 27.587 & 124.499\\
% ARMAX(2,3)-GARCH(1,1) & 25.004 & 30.523 & 34.317 & 127.979\\
% GBM                   & 13.899 & 13.722 & 16.028 & 131.899\\
% TME                   & 25.516 & 26.677 & 23.691 & 127.966\\
%   \hline
%   & MAE Q1 & MAE Q2 & MAE Q3 & MAE Q4 \\
%   \hline
% ARMA(2,3)-GARCH(1,1)  & 20.409 & 21.725 & 19.270 & 67.061\\
% ARMAX(2,3)-GARCH(1,1) & 19.737 & 21.970 & 19.885 & 70.435\\
% GBM                   & 11.453 &  9.786 & 12.265 & 76.158\\
% TME                   & 10.835 & 20.940 & 15.861 & 67.751\\
%   \hline
% \end{tabular}
% \end{center}
% \label{tab:10minQ1Q4}
% \end{table*}



% \begin{table}[!htbp]
% \begin{center}
%   \caption{Results of 1-min volume prediction.
%   The arrow symbols indicate the direction of the metrics for better models.
%   *Econometric models on Bitstamp market have numerical problems.}
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     \textbf{BITFINEX MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$\\
%     \hline
% ARMA(5,5)-GARCH(1,1)  & 24.547 & 14.227 & 2.660 & 117.348 \\
% ARMAX(5,5)-GARCH(1,1) & 24.629 & 14.189 & 2.664 & 117.084 \\
% GBM                   & 21.026 &  7.978 & NA    & NA \\
% TME                   & 20.142 & 10.204 & 2.654 & 44.344 \\
%     \hline
%     \hline
%     \textbf{BITSTAMP MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$\\
%     \hline
% *ARMA(6,4)-GARCH(1,1) & 1500.736 & 59.545 & 1.730 & 21700.844\\
% *ARMAX(6,4)-GARCH(1,1)& 293488.8274 & 9137.855 & 1.7223 & 266934176.5317\\
% GBM                   & 11.740   & 3.515  & NA    & NA\\
% TME                   & 11.378   & 4.299  & 1.721 & 10.295 \\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:1min}
% \end{table}

% \begin{table}[!htbp]
% \begin{center}
%   \caption{Results of 10-min volume prediction.
%   The arrow symbols in the first line indicate the direction of the metrics for better models.}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|}
%     \hline
%     \textbf{BITFINEX MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$ \\
%     \hline
% ARMA(5,4)-GARCH(1,1)  & 111.909 & 70.566 & 5.413 & 119.983\\
% ARMAX(5,4)-GARCH(1,1) & 111.794 & 69.912 & 5.397 & 118.020\\
% GBM                   & 110.197 & 61.506 & NA    & NA\\
% TME                   & 109.961 & 68.382 & 5.386 & 114.195\\
%     \hline
%     \hline
%     \textbf{BITSTAMP MARKET} & RMSE $\downarrow$ & MAE $\downarrow$ & NNLL $\downarrow$ & IW $\downarrow$ \\
%     \hline
% ARMA(2,3)-GARCH(1,1)  & 66.631 & 32.103 & 4.454 & 51.636 \\
% ARMAX(2,3)-GARCH(1,1) & 66.374 & 31.631 & 4.456 & 50.260 \\
% GBM                   & 67.128 & 27.719 & NA    & NA \\
% TME                   & 66.371 & 31.460 & 4.583 & 50.573 \\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:10min}
% \end{table}

%\tian{baselines leave or revise?}
%\subsection{Target variable -- processing}
% Let us denote $v_{i,l}$ the volume traded on day $l$ in an intraday time interval $i$, in units of Bitcoin. 
% For training dataset $\mathcal{D}^{\textit{train}}$, we extract the average intraday hourly patterns $\langle v_{h(i)} \rangle = \mathbb{E}_{l \thicksim \mathcal{D}^{\textit{train}}, i \thicksim h(i)}[v_{i,l} ]$
% , as the sample average over all intraday time minute intervals in specific hour $h(i)$ and training days.

% Next, to remove daily intraday hourly patterns, we process intraday volume in the following way: $w_{i,l} = \frac{v_{i,l}}{\langle v_{h(i)} \rangle}$. 
% Finally, the target variable we use are logarithmic values $u_{t}=\log(w_{i,l})$, where $t=(i,l)$ denotes the exact intraday interval and date time. 


